On the Effective Capacity of IRS-assisted wireless communication

We consider futuristic, intelligent reflecting surfaces (IRS)-aided communication between a base station (BS) and a user equipment (UE) for two distinct scenarios: a single-input, single-output (SISO) system whereby the BS has a single antenna, and a multi-input, single-output (MISO) system whereby the BS has multiple antennas. For the considered IRS-assisted downlink, we compute the effective capacity (EC), which is a quantitative measure of the statistical quality-of-service (QoS) offered by a communication system experiencing random fading. For our analysis, we consider the two widely-known assumptions on channel state information (CSI) -- i.e., perfect CSI and no CSI, at the BS. Thereafter, we first derive the distribution of the signal-to-noise ratio (SNR) for both SISO and MISO scenarios, and subsequently derive closed-form expressions for the EC under perfect CSI and no CSI cases, for both SISO and MISO scenarios. Furthermore, for the SISO and MISO systems with no CSI, it turns out that the EC could be maximized further by searching for an optimal transmission rate $r^*$, which is computed by exploiting the iterative gradient-descent method. We provide extensive simulation results which investigate the impact of the various system parameters, e.g., QoS exponent, power budget, number of transmit antennas at the BS, number of reflective elements at the IRS etc., on the EC of the system.

==> keywords.tex <==
\begin{keywords}

Effective capacity, D2D communication, Overlay, Inband, 5G

\end{keywords}} 

==> sec5.tex <==
\section{When CSIT is known to the Alice}
\label{sec:knownCSIT}
We consider the case as well when the CSIT is known to the Alice. In such scenario, we have $s_1$ and $s_3-s_5$ sates of the earlier defined states and the inequality of $s_1$ changes to equality. The state transition probability depends on the priors, false alarm and missed detection only. The service process $s_i(k)$ becomes different for $s_1$ only, the $s_i(k)$ is not a fixed number but is a random process here. Now we need to compute the MGF for this state. So, the MGF for $s_1$ is given as
\begin{align}
    E_{\gamma_i^A(k)}(e^{\theta s_i(k)})=\int_0^{\infty} e^{\theta s_i(k)} f_{\gamma_i^A(k)}(\gamma_i^A(k))d \gamma_i^A(k) \nonumber \\
      =  \int_0^{\infty} (1+\gamma_i^A(k))^{\frac{\theta}{\ln(2)}} f_{\gamma_i^A(k)}(\gamma_i^A(k))d \gamma_i^A(k)
\end{align}
%Solving the above equation is quite involved. Therefore, we solve it numerically (Using law of large number and Monte-Carlo based simulation)
Finally,  the $EC_i$ for known CSIT can be written as
\begin{align}
EC_i = \frac{1}{T+T_g} \big[\frac{-1}{\theta} \ln (\Pi(A)(1-P_{fa}). E_{\gamma_i^A(k)}(e^{-\theta s_i(k)})+p_3+p_4+p_5)
\end{align}
Knowing CSIT provides us benefit of enhancing EC of the system further through loading optimal power over sub-carriers.The formulated optimization program is given as
\begin{align}
\label{EC_opt}
\max_{P_i(H_i) \forall i} \ \ EC_T \\
\text{s.t} \ \ \sum_{i=1}^N P_i(H_i)\leqslant P_T  \nonumber \\
P_i(H_i)\geqslant 0 \ \ \forall i \nonumber
\end{align}
  The objective function is the sum of convex functions (hence convex itself) and the constraints $1$ and $2$ are linear (i.e convex sets). The two constraints ensure that total power allocation should not exceed $PT$ and the individual power should be positive. So, the program \ref{EC_opt} is indeed a convex program. We solve it through dual decomposition approach (with zero duality gap). The Dual program is given as
  \begin{align}
  \min_{\kappa \geq 0} \ \ D(\kappa)  
\end{align}  
where the dual function  $D(\kappa) $ is given as
\begin{align}
D(\kappa)= \max_{P_i(H_i)\geq 0 \forall i} L(\kappa,P_i(H_i) \forall i)
\end{align}
where $\kappa$ is the dual variable/Lagrangian multiplier and $L(.)=EC_T-\kappa (\sum_{i=1}^N P_i(H_i)$ is the Lagrangian function. After exploiting KKT conditions, we get the following for optimal power \cite{waqas:TETT:2018}
 \begin{align}
 P_i(H_i)^{\ast}= \left( \frac{\frac{\theta}{\ln(2)}+1}{\kappa \Pi(A)(1-P_{fa}) }-\frac{1}{\vert H_i \vert^2}\right)^+ 
 \end{align}
 Next, we remain to solve the dual problem, we solve it through sub-gradient method given as
 \begin{align}
 \kappa(m)=\kappa(m-1)-\alpha\left(PT-\sum_{i=1}^N P_i(H_i)^{\ast}\right)
 \end{align}
 where $m$ is the iteration and $\alpha$ is the step size. This completes the solution to problem \ref{EC_opt}
%\begin{align}
% P_i^\ast(H_i)&=\begin{cases}
%\left(C^\dagger-\vert H_i\vert^2\right)\frac{1}{(\vert H_i\vert^2)^{\frac{\theta}{\ln(2)}+1}}, &  if C^\dagger \geq\vert H_i\vert^2 \nonumber \\
%\\
%0, &  \text{otherwise}.
%\end{cases}
%\end{align}
%where $C`=(\frac{\kappa \ln(2)}{\Pi(A)(1-P_{fa})\theta } )^{\frac{\theta}{\ln(2)}+1}$, $\kappa$ is the Lagrangian multiplier and we find its value by the use of constraint 1 and as given as
%\begin{align}
%  C^\dagger =\frac{\sum_{i=1}^N\frac{1}{\vert H_i\vert^2}}{\sum_{i=1}^N\frac{1}{(\vert H_i\vert^2)^{\frac{\theta}{\ln(2)}+1}}}
%  \end{align}
%  \begin{align}
%  P_i^\ast(H_i)=\left((\frac{\kappa \ln(2)}{\Pi(A)(1-P_{fa})\theta \vert H_i\vert^2 } )^{\frac{\theta}{\ln(2)}+1}-\frac{1}{\vert H_i\vert^2}\right)^+
%  \end{align}

  
  
%  \begin{align}
%
%P_i^\ast(H_i)=
%\end{align}
%\\
%\textcolor{red}{In such scenario, the service process $s_i(k)$ is no more Bernoulli random variable.   The maximum arrival $r^*$ in such case is given as [Soret et al]
%\begin{equation}
%    r^*=0.5. E\{s_i\}+0.5\sqrt{(E\{s_i \})^2+2\frac{2.ln(p_d)}{d}\sigma_{s_i}^2}
%\end{equation}
%Here, we need to find the first and second moment of random variable $s_i$. So, $s_i= \Delta f \log_2(1+\gamma_i^A)$. Now
%\begin{equation}
% E\{s_i\}=\Delta f \int_{0}^{\infty} \log_2(1+\gamma_i^A)f_{\gamma_i^A} d_{\gamma_i^A}    
%\end{equation}
%Similarly
%\begin{equation}
% \sigma_{s_i}^2=2\Delta f^2 \int_{0}^{\infty} \log_2(1+\gamma_i^A)f_{\gamma_i^A} d_{\gamma_i^A}    
%\end{equation}
%}
